Resource Optimization with Flexible Numerology and Frame Structure for Heterogeneous Services

We explore the potential of optimizing resource allocation with flexible numerology in frequency domain and variable frame structure in time domain, in presence of services with different types of requirements. We analyze the computational complexity and propose a scalable optimization algorithm based on searching in both the primal space and dual space that are complementary to each other. Numerical results show significant advantages of adopting flexibility in both time and frequency domains for capacity enhancement and meeting the requirements of mission critical services.

==> macro.tex <==
\usepackage{acronym}
%\pgfplotsset{compat=1.15}
                         %
\newcommand{\todo}[1]
{\iftodo
  \iftodoshort
  \reversemarginpar\marginpar{\textdbend \sf\scriptsize ToDo}
  [.1em]\par
  \else
  \reversemarginpar\marginpar{\textdbend \sf\scriptsize ToDo}
  \noindent
  \fbox{\begin{minipage}[c]{0.95\linewidth}
       {\color{blue}{\small #1}}
    \end{minipage}     
  }
  \\[.1em]\par
  \fi % todoshort
  \fi}
	
%\usepackage[normalem]{ulem}
%\newcommand{\inQL}[1]{\textcolor{blue}{#1}}
%\newcommand{\reQL}[1]{\textcolor{red}{\sout{#1}}}
%\newcommand{\coQL}[1]{\textbf{{\textcolor{green}{(Comment [QL]: #1)}}}}

\newcommand{\inQL}[1]{#1}
\newcommand{\reQL}[1]{}
\newcommand{\coQL}[1]{}



==> model.tex <==
% Qi's part on system model
\subsection{Design of Blocks}
Comparing to \ac{LTE} that applies a fixed \ac{SCS} of $15$ kHz and \ac{TTI} of $0.5$ ms, \ac{5G}/\ac{NR} will support scalable numerologies and frame structures \cite{3GPP38802}. A large set of block shapes are suggested in \cite{3GPP38802} with numerology varying from 15 kHz to 480 kHz, and \ac{TTI} duration varying from 0.125 ms to 0.5 ms. In this paper, we consider $4$ most widely accepted block shapes, provided in Table \ref{tab:numerology}. Note that Shape 3E supports extended \ac{CP} length to trade off overhead against delay spread.
%
\begin{table}[!h]
\centering
\caption{Selected candidate blocks}
\begin{tabular}{lllll}
\toprule
\textbf{} & \textbf{Shape 1} & \textbf{Shape 2} & \textbf{Shape 3} & \textbf{Shape 3E} \\
TTI duration (ms) & $0.5$ & $0.25$ & $0.125$ & $0.125$\\ 
SCS (kHz) & $15$ & $30$ & $60$ & $60$ \\
Symbol duration ($\mu$s) & $66.7$ & $33.3$ & $16.7$ & $16.7$ \\
CP ($\mu$s) & $4.7$ & $2.3$ & $1.2$ & $4.17$ \\
Number of symbols & $7$ & $7$ & $7$ & $6$ \\
\bottomrule
\end{tabular}
\label{tab:numerology} 
\end{table}
%
\subsection{Modeling Per-Block Capacity}

Given channel profile, transmission power, and noise power over communication link of service $k$, the capacity $r_{b,k}$ depends on the configuration of block $b$, including time span and frequency range (characterized by \ac{SCS} and \ac{TTI} duration), \ac{CP} length, and symbol duration. We assume a $9$ multipath channel profile \cite[Table B.2.2.1-4]{3GPP36803}, and predefine the mapping from a tuple consisting of channel profile, transmission power, noise power, and block configuration to the block capacity based on the model introduced in \cite{batariere2004cyclic}. 

%Due to limited space, and the fact that modeling capacity is not in the scope of this paper, we omit the details but provide the tutorial and source code in \href{https://github.com/youlei202/Flexible_TTI}{a public repository on GitHub} \cite{githublink}.


==> paper(double_column)/acronyms.tex <==
\acrodef{3GPP}{3rd generation partnership project}
\acrodef{5G}{fifth generation}
% A
 \acrodef{ABS}{almost blank subframe}
% B
    \acrodef{BS}{base station}
% C
    \acrodef{CDF}{cumulative distribution function}
    \acrodef{CSI}{channel state information}
    \acrodef{CQI}{channel quality indicator}
		\acrodef{CP}{cyclic prefix}
% D
\acrodef{DL}{downlink}
    \acrodef{DUDe}{downlink and uplink decoupling}
% E
\acrodef{eICIC}{enhanced intercell interference coordination}
\acrodef{ESD}{energy spectral density}
% F
\acrodef{FDD}{frequency division duplex}
    \acrodef{FDMA}{frequency division multiple access}
% G
   \acrodef{GP}{Gaussian process}
    \acrodef{GPS}{global positioning system}
% H
\acrodef{HetNet}{heterogeneous network}
% I 
    \acrodef{ICI}{inter-cell interference}
		\acrodef{IMI}{inter-mode interference}
		\acrodef{ISI}{inter-symbol interference}
% J
% K
% L
\acrodef{LTE}{long term evolution}

% M
\acrodef{MAC}{media access control}
\acrodef{MRU}{minimum resource unit}
% N
\acrodef{NR}{new radio}

% O
   \acrodef{OFDM}{orthogonal frequency division multiplexing}
% P
    \acrodef{PDF}{probability density function}
    \acrodef{PHY}{physical layer}
		\acrodef{PSD}{power spectral density}
    \acrodef{PRB}{physical resource block}
		\acrodef{RU}{resource unit}
% Q
   \acrodef{QoE}{quality of experience}
    \acrodef{QoS}{quality of service}
% R
    \acrodef{RAN}{radio access network}
		\acrodef{RBS}{removal of bottleneck services}
		\acrodef{RMDI}{resource muting for dominant interferer}
    \acrodef{RRM}{radio resource management}
		\acrodef{RU}{resource unit}
		\acrodef{RX}{receiver}
% S
 \acrodef{SAFP}{successive approximation of fixed point}
    \acrodef{SDN}{software defined network}
    \acrodef{SNR}{signal-to-noise ratio}
    \acrodef{SINR}{signal-to-interference-plus-noise ratio}
\acrodef{SIR}{signal-to-interference ratio}
\acrodef{SIF}{standard interference function}
    \acrodef{SVM}{support vector machine}
		\acrodef{SCS}{sub-carrier spacing}
% T
    \acrodef{TCP}{transmission control protocol}
		\acrodef{TDD}{time division duplex}
    \acrodef{TDMA}{time division multiple access}
		\acrodef{TTI}{transmission time interval}
		\acrodef{TX}{transmitter}
		% U 
		\acrodef{UE}{user equipment}
		\acrodef{UL}{uplink}
		% V
		% W
    \acrodef{WLAN}{wireless local area network}
% X
% Y 
% Z

==> paper(double_column)/macro.tex <==
\usepackage{acronym}
%\pgfplotsset{compat=1.15}
                         %
\newcommand{\todo}[1]
{\iftodo
  \iftodoshort
  \reversemarginpar\marginpar{\textdbend \sf\scriptsize ToDo}
  [.1em]\par
  \else
  \reversemarginpar\marginpar{\textdbend \sf\scriptsize ToDo}
  \noindent
  \fbox{\begin{minipage}[c]{0.95\linewidth}
       {\color{blue}{\small #1}}
    \end{minipage}     
  }
  \\[.1em]\par
  \fi % todoshort
  \fi}
	
%\usepackage[normalem]{ulem}
%\newcommand{\inQL}[1]{\textcolor{blue}{#1}}
%\newcommand{\reQL}[1]{\textcolor{red}{\sout{#1}}}
%\newcommand{\coQL}[1]{\textbf{{\textcolor{green}{(Comment [QL]: #1)}}}}

\newcommand{\inQL}[1]{#1}
\newcommand{\reQL}[1]{}
\newcommand{\coQL}[1]{}



==> paper(double_column)/model.tex <==
% Qi's part on system model
\subsection{Design of Blocks}
Comparing to \ac{LTE} that applies a fixed \ac{SCS} of $15$ kHz and \ac{TTI} of $0.5$ ms, \ac{5G}/\ac{NR} will support scalable numerologies and frame structures \cite{3GPP38802}. A large set of block shapes are suggested in \cite{3GPP38802} with numerology varying from 15 kHz to 480 kHz, and \ac{TTI} duration varying from 0.125 ms to 0.5 ms. In this paper, we consider $4$ most widely accepted block shapes, provided in Table \ref{tab:numerology}. Note that Shape 3E supports extended \ac{CP} length to trade off overhead against delay spread.
%
\begin{table}[!h]
\centering
\caption{Selected candidate blocks}
\begin{tabular}{lllll}
\toprule
\textbf{} & \textbf{Shape 1} & \textbf{Shape 2} & \textbf{Shape 3} & \textbf{Shape 3E} \\
TTI duration (ms) & $0.5$ & $0.25$ & $0.125$ & $0.125$\\ 
SCS (kHz) & $15$ & $30$ & $60$ & $60$ \\
Symbol duration ($\mu$s) & $66.7$ & $33.3$ & $16.7$ & $16.7$ \\
CP ($\mu$s) & $4.7$ & $2.3$ & $1.2$ & $4.17$ \\
Number of symbols & $7$ & $7$ & $7$ & $6$ \\
\bottomrule
\end{tabular}
\label{tab:numerology} 
\end{table}
%
\subsection{Modeling Per-Block Capacity}

Given channel profile, transmission power, and noise power over communication link of service $k$, the capacity $r_{b,k}$ depends on the configuration of block $b$, including time span and frequency range (characterized by \ac{SCS} and \ac{TTI} duration), \ac{CP} length, and symbol duration. We assume a $9$ multipath channel profile \cite[Table B.2.2.1-4]{3GPP36803}, and predefine the mapping from a tuple consisting of channel profile, transmission power, noise power, and block configuration to the block capacity based on the model introduced in \cite{batariere2004cyclic}. 

%Due to limited space, and the fact that modeling capacity is not in the scope of this paper, we omit the details but provide the tutorial and source code in \href{https://github.com/youlei202/Flexible_TTI}{a public repository on GitHub} \cite{githublink}.

